Energy-Based Test Sample Adaptation for Domain Generalization

In this paper, we propose energy-based sample adaptation at test time for domain generalization. Where previous works adapt their models to target domains, we adapt the unseen target samples to source-trained models. To this end, we design a discriminative energy-based model, which is trained on source domains to jointly model the conditional distribution for classification and data distribution for sample adaptation. The model is optimized to simultaneously learn a classifier and an energy function. To adapt target samples to source distributions, we iteratively update the samples by energy minimization with stochastic gradient Langevin dynamics. Moreover, to preserve the categorical information in the sample during adaptation, we introduce a categorical latent variable into the energy-based model. The latent variable is learned from the original sample before adaptation by variational inference and fixed as a condition to guide the sample update. Experiments on six benchmarks for classification of images and microblog threads demonstrate the effectiveness of our proposal.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/Table1.tex <==
\linespread{1.2}
\begin{table}[!h]
\centering
\caption{\textbf{Comparison with baseline models on PASCAL VOC 2012.} We implement all models using the same hyperparameters and protocols. Mean value and variance are reported after three runs. Our model is a consistent top-performer.}
\resizebox{5in}{!}{
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{6}{c}{\textbf{PASCAL VOC 2012}}  \\
\multicolumn{1}{c}{}                       & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{7-shot} & \textbf{9-shot} & \textbf{mean} \\ \midrule
O-MN                                       & 51.60 \scriptsize{$\pm$  2.11}      & 53.82 \scriptsize{$\pm$ 4.68}      & 53.62 \scriptsize{$\pm$ 3.16}      & 53.10 \scriptsize{$\pm$ 1.17}        & 51.94 \scriptsize{$\pm$ 3.36}       &  52.62 \scriptsize{$\pm$ 0.03}    \\
O-PN                                       & 52.63 \scriptsize{$\pm$ 3.74}      &  57.96 \scriptsize{$\pm$ 2.61}      &  59.30 \scriptsize{$\pm$ 1.89}      & 59.53 \scriptsize{$\pm$ 0.10}       &   58.60 \scriptsize{$\pm$ 1.51}     &  57.55 \scriptsize{$\pm$ 0.05} \\
O-APN         & 54.14 \scriptsize{$\pm$ 1.17}       & 57.30 \scriptsize{$\pm$ 2.55}       & 58.12 \scriptsize{$\pm$ 2.29}       &  58.45 \scriptsize{$\pm$ 0.75}   &57.13 \scriptsize{$\pm$ 1.25}   & 56.76 \scriptsize{$\pm$ 0.02} \\
LSTM        & 55.40 \scriptsize{$\pm$ 2.79}      & 58.96 \scriptsize{$\pm$ 3.36}       & 59.63 \scriptsize{$\pm$ 0.74}       &    60.03 \scriptsize{$\pm$ 0.22}   & 58.50 \scriptsize{$\pm$ 0.17}    & 58.29 \scriptsize{$\pm$ 0.10}   \\
\rowcolor[gray]{.9}\textbf{Ours}                                           & \textbf{59.41} \scriptsize{$\pm$ 2.50}      & \textbf{62.82} \scriptsize{$\pm$ 2.31}    & \textbf{62.91} \scriptsize{$\pm$ 1.29}       & \textbf{62.91} \scriptsize{$\pm$ 0.16}       & \textbf{61.73} \scriptsize{$\pm$ 2.16}      & \textbf{61.83} \scriptsize{$\pm$ 0.10} \\ 
\bottomrule
\end{tabular}}
\label{pascal}
\end{table}

%Offline-1                                  &  53.62 \scriptsize{$\pm$ 0.03     & 53.91 \scriptsize{$\pm$ 0.03      & 53.40 \scriptsize{$\pm$ 0.31       & 53.53 \scriptsize{$\pm$ 0.24       &  53.33 \scriptsize{$\pm$ 0.03      & 53.51 \scriptsize{$\pm$ 0.04\\
%Offline-5                                  & 54.47 \scriptsize{$\pm$ 0.05     & 56.87 \scriptsize{$\pm$ 0.01    &  57.18 \scriptsize{$\pm$ 0.02      & 57.43 \scriptsize{$\pm$ 0.02       &  57.57 \scriptsize{$\pm$ 0.05    & 56.91 \scriptsize{$\pm$ 0.01   \\

==> table/Table2.tex <==
\linespread{1.2}
\begin{table}[!h]
\centering
\caption{\textbf{Comparison with baseline models on COCO.} We implement all models using the same hyperparameters and protocols. Mean value and variance are reported after three runs. Our model is a consistent top-performer.}
\resizebox{5in}{!}{
\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{6}{c}{\textbf{COCO}}  \\
\multicolumn{1}{c}{}                       & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{7-shot} & \textbf{9-shot} & \textbf{mean} \\ \hline
O-MN                        & 23.4$\pm$4.18      & 22.42$\pm$0.68       & 21.73$\pm$0.07        & 23.30$\pm$3.83       &  22.48$\pm$0.03   &22.84 $\pm$0.78 \\
O-PN              &  39.59$\pm$1.87    & 42.60$\pm$1.40     & 45.22$\pm$0.36       &   45.11$\pm$0.39     &  47.06$\pm$3.40  & 44.22$\pm$0.20\\
O-APN         & 35.36$\pm$5.46      & 36.83$\pm$3.19      & 37.99$\pm$1.87      &  38.49$\pm$4.18   &40.42$\pm$3.20   & 38.19$\pm$0.66 \\
LSTM        &35.52$\pm$1.89      & 41.45$\pm$3.32       & 44.65$\pm$1.36       &   45.67$\pm$0.55   & 47.71$\pm$5.13    & 43.84$\pm$0.58   \\
    \rowcolor[gray]{.9} \textbf{Ours}                                           & \textbf{43.08$\pm$1.61}      & \textbf{45.96$\pm$1.18}    & \textbf{49.17$\pm$0.5}       & \textbf{48.30$\pm$0.14}       & \textbf{49.93$\pm$3.24}      & \textbf{47.79$\pm$0.29} \\ \hline
\end{tabular}}
\label{coco}
\end{table}

%Offline-1                                  &  33.38$\pm$1.36     & 38.42$\pm$0.40      & 38.06$\pm$0.91       & 39.78$\pm$1.14       &  38.63$\pm$2.15      & 38.13$\pm$0.15\\
%Offline-5               & 38.76$\pm$1.55    &  43.09$\pm$0.20      & 43.90$\pm$0.43       &  45.26$\pm$0.77    & 44.08$\pm$1.96   &43.64$\pm$0.28 \\

==> table/Table3.tex <==
\linespread{1.2}
\begin{table}[!h]
\centering
\caption{\textbf{Comparison with baseline models on ABD-MR-20.} We implement all models using the same hyperparameters and protocols. Mean value and variance are reported after three runs. Our model is a consistent top-performer.}
\resizebox{5in}{!}{
\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{6}{c}{\textbf{ABD-MR-20}}  \\
\multicolumn{1}{c}{}                       & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{7-shot} & \textbf{9-shot} & \textbf{mean} \\ \hline
O-MN                       & 11.58$\pm$2.24      & 30.54$\pm$1.16       & 41.81$\pm$1.15       & 35.52$\pm$0.29       &  17.45$\pm$1.18   & 26.86$\pm$0.36 \\
O-PN              &  16.95$\pm$1.27    & 36.73$\pm$0.23     & 50.22$\pm$0.36       &  43.54$\pm$0.01     &  26.85$\pm$0.29  & 34.21$\pm$0.08 \\
O-APN         & 14.74$\pm$1.81      &34.13$\pm$0.20      & 51.37$\pm$0.28      &  48.44$\pm$1.03   &29.38$\pm$0.74   & 35.34$\pm$0.23 \\
LSTM        &13.36$\pm$1.40      & 31.92$\pm$0.10       & 44.85$\pm$0.23       &   46.15$\pm$1.55   & 27.98$\pm$0.80   & 31.66$\pm$0.18   \\
    \rowcolor[gray]{.9} \textbf{Ours}                                           & \textbf{13.74$\pm$0.58}      & \textbf{37.02$\pm$0.61}    & \textbf{54.98$\pm$0.09}       & \textbf{54.10$\pm$0.71}       & \textbf{38.24$\pm$2.05}      & \textbf{38.56$\pm$0.28} \\ \hline
\end{tabular}}
\label{coco}
\end{table}

==> table/classifier.tex <==
\linespread{1.15}
\begin{table}[!h]
\caption{\textbf{Learnable classifier vs. adaptive classifier on Online-PASCAL.} Variational adaptive classifier is  more critical than naive adaptive classifier and learnable classifier for online few-shot segmentation.}
\centering
\resizebox{5.5in}{!}{\begin{tabular}{lcccccc}
\hline
\textbf{Method}     & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{7-shot} & \textbf{9-shot} & \textbf{mean} \\
Learnable classifier   & 54.25$\pm$1.75       &    58.23$\pm$2.38   & 59.41$\pm$1.17        & 59.81$\pm$0.69       & 58.41$\pm$1.48       &  57.82$\pm$0.04    \\
Naive adaptive classifier & 57.86$\pm$3.56       &  61.79$\pm$2.86   & 61.93$\pm$1.72        & 62.38$\pm$0.11       & 61.14$\pm$1.29       &  60.94$\pm$0.11    \\
\rowcolor[gray]{.9} \textbf{Variational adpative classifier}                                           & \textbf{59.41$\pm$2.50}      & \textbf{62.82$\pm$2.31}    & \textbf{62.91$\pm$1.29}       & \textbf{62.91$\pm$0.16}       & \textbf{61.73$\pm$2.16}      & \textbf{61.83$\pm$0.10}\\ \hline
\label{classifier}
\end{tabular}}
\vspace{-3mm}
\end{table}

==> table/fold.tex <==
\linespread{1}
\begin{table}[!h]
\caption{\textbf{Cross validation on different unseen classes.} For each fold, testing samples come from different unseen classes.}
\centering
\resizebox{5.5in}{!}{\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Online-PASCAL}} & \multicolumn{4}{c}{\textbf{Online-COCO}}   \\
                        & \textbf{Fold-0} & \textbf{Fold-1} & \textbf{Fold-2} & \textbf{Fold-3} & \textbf{Fold-0} & \textbf{Fold-1} & \textbf{Fold-2} & \textbf{Fold-3} \\
baseline(lrcls)                   & 57.82$\pm$0.04       & 66.15$\pm$0.26       & 52.35$\pm$0.12      & 49.66$\pm$0.26       & 41.74$\pm$0.36        & 37.23$\pm$0.24       & 16.43$\pm$0.45       & 25.20$\pm$0.37       \\
\rowcolor[gray]{.9} \textbf{Ours}                    &  61.83$\pm$0.10      &  68.87$\pm$0.31      & 53.17$\pm$0.05       & 51.46$\pm$0.32       & \textbf{47.79$\pm$0.29}       & 41.14$\pm$0.38       &18.63$\pm$0.11        & 27.60$\pm$0.42       \\ \hline
\end{tabular}}
\label{fold}
\end{table}

==> table/memory.tex <==
\linespread{1.15}
\begin{table}[!t]
\caption{\textbf{Benefits of external memory.} The experiments are conducted on Online-PASCAL using ResNet50 averaged over three runs. With the external memory (the second row), the method achieves significant performance.}
\centering
\resizebox{5in}{!}{\begin{tabular}{lcccccc}
\hline
\textbf{Method}     & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{7-shot} & \textbf{9-shot} & \textbf{mean} \\
w/o External memory & 57.10$\pm$2.84       &    58.37$\pm$1.33    & 58.23$\pm$1.65        & 57.48$\pm$0.15       & 56.67$\pm$1.62       &  57.23$\pm$0.14    \\
\rowcolor[gray]{.9} \textbf{External memory}            & \textbf{59.41$\pm$2.50}      & \textbf{62.82$\pm$2.31}    & \textbf{62.91$\pm$1.29}       & \textbf{62.91$\pm$0.16}       & \textbf{61.73$\pm$2.16}      & \textbf{61.83$\pm$0.10}\\ \hline
\label{memory}
\end{tabular}}
\vspace{-5mm}
\end{table}

==> table/prior.tex <==
\linespread{1.15}
\begin{table}[!t]
\caption{\textbf{Benefits of two priors described in Eq. (\ref{model}) and Eq. (\ref{ELBO2}).} With the prior conditioned on current sample $x_t$ and external memory $\mathcal{M}_t$, the method achieves better performance than with prior conditioned only on external memory $\mathcal{M}_t$.}
\centering
\resizebox{5in}{!}{\begin{tabular}{lcccccc}
\hline
\textbf{Prior}     & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{7-shot} & \textbf{9-shot} & \textbf{mean} \\
$p(\theta_t|\mathcal{M}_t)$ Eq. (\ref{model}) & 54.84$\pm$1.37       &    58.96$\pm$2.87   & 60.03$\pm$0.78        & 60.30$\pm$0.39       & 59.11$\pm$0.96       &  58.53$\pm$0.18    \\
\rowcolor[gray]{.9} \textbf{$p(\theta_t|x_t,\mathcal{M}_t)$ Eq. (\ref{ELBO2})}                                          & \textbf{59.41$\pm$2.50}      & \textbf{62.82$\pm$2.31}    & \textbf{62.91$\pm$1.29}       & \textbf{62.91$\pm$0.16}       & \textbf{61.73$\pm$2.16}      & \textbf{61.83$\pm$0.10}\\ \hline
\label{prior}
\end{tabular}}
\vspace{-8mm}
\end{table}
